Recognizing Developers' Emotions while Programming

Developers experience a wide range of emotions during programming tasks, which may have an impact on job performance. In this paper, we present an empirical study aimed at (i) investigating the link between emotion and progress, (ii) understanding the triggers for developers' emotions and the strategies to deal with negative ones, (iii) identifying the minimal set of non-invasive biometric sensors for emotion recognition during programming task. Results confirm previous findings about the relation between emotions and perceived productivity. Furthermore, we show that developers' emotions can be reliably recognized using only a wristband capturing the electrodermal activity and heart-related metrics.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}
During their daily work, developers experience~\cite{MF15,Serebrenik17:benevol} and share~\cite{MurgiaTAO14} a wide range of emotions. 
Current research is studying the link between such emotions and performance~\cite{GraziotinWA15:Journal,GraziotinFWA18:JSS,GraziotinWA13:PROFES,MF15,Khan2011}.
Some studies focus on understanding the triggers for unhappiness and frustration in software development ~\cite{GraziotinFWA17, FordP15:CHASE}, while others assess the impact of time pressure on productivity and software quality~\cite{Kuutila:survey}. 

% In this vein, we envision the emergence of tools supporting emotion recognition and awareness during software development.   
%In this context, awareness of one's own and fothers' emotions is the first step towards developing emotional intelligence, that is the ability to perceive and express emotion, assimilate emotion in thought, understand and reason with emotion, and regulate emotion in the self and others [19].

In a software company, emotion awareness is beneficial at different levels of aggregation to enable implementation of best practices and early detection and resolution of problems, thus decreasing the risk of burnout and undesired turnover~\cite{MantylaADGO16}. For example, Microsoft includes consideration of emotions for inclusive hiring and to support neuro-diverse developers~\cite{MorrisBW15}.
Similarly, information about developers' emotional state can be leveraged to evaluate collaborative software development strategies~\cite{Guzman:2013}. 

In a company that promotes and applies Agile development, the ability to identify developers' negative emotions, such as stress~\cite{} and frustration~\cite{FordP15:CHASE} can be used as a proxy to discover that agile principles are not being applied correctly or that developers are not aligned with such principles. Indeed, recent research findings~\cite{FordP15:CHASE} demonstrate how negative emotions may be caused by uneven task distribution due to wrong estimation of size or time required to complete an assignment, by difficulties experienced by a team member in solving a complex cognitive task, or in the presence of obstacles when getting familiar with a new technology or programming language. Thus, managers and Scrum masters can benefit from enriching retrospective meeting with emotional feedback collected from the developers~\cite{Zanchi}. 

At the level of individuals, increasing developers' self-awareness of own emotions can be beneficial to improve  productivity and enhance resilience to failures.
In such a scenario, we envisage the development of tools for early detection of developers' negative emotions associated with poor job performance, such as stress~\cite{MantylaADGO16}, frustration~\cite{FordP15:CHASE}, and anger~\cite{GachechiladzeLN17} to suggest developers corrective actions.

The work of Graziotin et al.~\cite{GraziotinWA13:PROFES,GraziotinWA15:Journal} shows [QUICK SUMMARY OF GRAZIOTIN CONTRIBUTIONS] whereas M\"uller and Fritz~\cite{MF15} shows [QUICK SUMMARY OF FRITZ CONTRIBUTIONS]. 
In the study reported in this paper, we define research questions and study design based on Graziotin et al.~\cite{GraziotinWA13:PROFES,GraziotinWA15:Journal}  
 and M\"uller and Fritz~\cite{MF15}. 
%during programming tasks. 
%seek to confirm and extend the findings of two previous researches  and  
In particular, the first goal of this paper is to investigate the link between emotions of software developers and their perceived productivity.

Hence, we formulate our first research question as follows: 
\begin{itemize}
    \item \textit{RQ1} - What is the range of developers' emotions during a programming task and to what extent they correlate with their perceived progress? 
\end{itemize}
M\"uller and Fritz shows that [HIGHLIGHT RESULTS], however, [SAY HOW WE DO IT DIFFERENTLY/BETTER].
A repeated measurements design is conducted with 23 participants involved in a programming task replicated from the study by M\"uller and Fritz~\cite{MF15}.
The analysis of the correlation between self-reported emotions and progress was performed by fitting s linear-mixed effect model

Software developers experience a wide range of emotions which can divided into positive and negative ones.
In this study, we are interested in differentiating them and  identifying coping strategies for dealing with negative emotions.
We formulate our second research question: 
\begin{itemize}
    \item \textit{RQ2} - What are the triggers for developers' emotions and the strategies developers implement to deal with such negative ones? 
\end{itemize}
Graziotin et al. shows that [HIGHLIGHT RESULTS], however, [SAY HOW WE DO IT BETTER].
We perform manual coding of participants' answers to open-ended questions to understand the causes of emotions and the strategies to deal with them.

To tackle the above research questions, we use biometrics sensors~\cite{MF15} [QUICK DESCRIPTION].
% Previous work~\cite{MF15} demonstrated the feasibility of emotion detection based on  biometric sensors during programming tasks.
To simplify experimental settings in further studies (e.g., gathering and cleaning less data, removing useless features, and improve the ecological validity), we aim at identifying the minimal set of sensors to wear in the work environment for our results to be applicable.
Accordingly, we formulate our third research question:
%Nowadays, emotion recognition based on biometrics is a consolidated research field~\cite{KimA08,KoelstraMSLYEPNP12,SoleymaniAFP16}. However, the biometric sensors usually employed in a laboratory setting can be expensive or uncomfortable to wear in a natural setting such as the work environment. As such, other than confirming previous findings by M\"uller and Fritz~\cite{MF15} about the feasibility of sensor-based emotion recognition during software development, we also aim at assessing the reliability of low-cost noninvasive devices. 

%We operationalize emotions in term of (un)pleasantness of the stimulus (\textit{valence}) and the level of activation (\textit{arousal}), according to the Circumplex Model proposed by Russell~\cite{JS1980}. As such, we formulate our third research question as follows:

%  \begin{itemize}
%  \item \textit{RQ3} -  Can we use noninvasive, low cost biometric sensors to determine developers' emotions during a programming task?
%  \end{itemize}
%In addition to previous work,  Hence, we specify RQ3 as follows:
  \begin{itemize}
  \item \textit{RQ3} - What is the minimal set of non-invasive biometric sensors to recognize developers' emotions during a programming task?
\end{itemize}
Supervised machine learning is used to train a classifier for emotional valence and arousal using features based on biometrics with different sensor configurations. 
% To address our research questions we leverages a mix of qualitative and quantitative methods.

The contributions of this work are:
\begin{itemize}
    \item A set of machine learning models to classify developers emotions during a programming tasks.
    \item An experimental protocol for the collection and analysis of biometric-based data from software developers.
    \item A lab package to verify the results and replicate this study. 
\end{itemize}

The reminder of the paper is structured as follows: ...


==> sections/introduction_new.tex <==
\section{Introduction}
\label{sec:introduction}
%During their daily work, software developers experience~\cite{MF15,Serebrenik17:benevol} and share~\cite{MurgiaTAO14} a wide range of both positive and negative emotions.
%Supporting developers' self-awareness of own emotions is beneficial to improve their productivity and enhance resilience to failures. 
Software development is an intellectual activity requiring creativity and problem-solving skills, which are influenced by affective states~\cite{GWA14}.  
Previous work shows that positive emotions are beneficial for developers' well-being and productivity while negative ones lead to poor job performance and are detrimental to the software development process~\cite{GraziotinFWA18:JSS, Khan2011, MF15}. 
Hence, emotion awareness---i.e, the awareness of own and others' emotions---is regarded as a key to success for software projects~\cite{Denning:2012}. 

Early recognition of negative emotions, such as stress~\cite{MantylaADGO16}, frustration~\cite{FordP15:CHASE}, and anger~\cite{GachechiladzeLN17} can enable just-in-time corrective actions for developers and team managers, preventing burnout and undesired turnover~\cite{MantylaADGO16}. 
Recent research findings demonstrate that negative emotions can be caused by uneven task distribution, wrong estimation of size and time required to complete an assignment,  difficulties solving a complex cognitive task, and obstacles when familiarizing with a new technology or programming language~\cite{FordP15:CHASE}. 
%Managers can provide support when developers are stuck~\cite{Holman18} by re-establishing mental well-being and making them productive again. 
Information about developers' emotional state can be leveraged to improve collaborative software development strategies~\cite{Guzman:2013}.
For instance, enriching retrospective meetings with feedback about developers' emotions can be used to reflect as a team on opportunities for improvement.
Thus, we envision the emergence and adoption of tools for enhancing emotion awareness during software development. 

In this study, we focus on the identification of the emotions experienced by developers engaged in a programming task. Specifically, we operationalize emotions along the valence and arousal dimensions of the Circumplex Model of affect~\cite{JS1980}.
First, we build upon recent research investigating the relation between developers' emotions and perceived productivity~\cite{GraziotinWA15:Journal, MF15}.
We formulate our first research question as follows:
\begin{adjustwidth}{0.7cm}{}
\textit{RQ1} - What is the range of developers' emotions during a programming task and to what extent they correlate with their perceived progress?
\end{adjustwidth}
To address RQ1, we perform a study with 23 participants engaged in a programming task. 
We ask participants to periodically self-report their emotional state and self-assessed progress.
We analyze the range of emotions reported and their correlation with perceived progress by fitting a linear-mixed effect model as done in the previous studies~\cite{MF15, GraziotinWA15:Journal}.

As a second goal, we aim at discovering the causes of positive and negative emotions experienced during software development. 
Furthermore, we aim at identifying the coping strategies that might help programmers dealing with negative emotions.
As such, we formulate our second research question: 
\begin{adjustwidth}{0.7cm}{}
\textit{RQ2} - What are the triggers for developers' emotions and the strategies they implement to deal with negative ones?
\end{adjustwidth}
To address RQ2, we interview the participants at the end of the study and perform manual coding~\cite{Martin:Turner} of their answers to open-ended questions. 

%Finally, we aim at enhancing the state-of-the-art on developers' emotion detection using wearable biometric sensors. 
% Finally, we aim explore the use of wearable biometric sensors to detect developers' emotions in their daily work. 
Previous work demonstrated the feasibility of sensor-based emotion detection using non-invasive biometric devices~\cite{MF15, Girardi:ACII2017}.
However, the experimental setting usually employed in a laboratory setting is too complex for being applied in practice. 
We aim at identifying the minimal set of sensors to wear in the work environment for reliable emotion recognition.
Accordingly, we formulate our third research question:
%Nowadays, emotion recognition based on biometrics is a consolidated research field~\cite{KimA08,KoelstraMSLYEPNP12,SoleymaniAFP16}. However, the biometric sensors usually employed in a laboratory setting can be expensive or uncomfortable to wear in a natural setting such as the work environment. As such, other than confirming previous findings by M\"uller and Fritz~\cite{MF15} about the feasibility of sensor-based emotion recognition during software development, we also aim at assessing the reliability of low-cost noninvasive devices. 
\begin{adjustwidth}{0.7cm}{}
\textit{RQ3} - What is the minimal set of non-invasive biometric sensors to recognize developers' emotions?
\end{adjustwidth}
We use supervised machine learning to train a classifier for developers' emotions based on biometric features, with different sensor configurations. 
% To address our research questions we leverages a mix of qualitative and quantitative methods.

The contributions of this work are:
\begin{itemize}
    \item A list of emotional triggers related to software development, including strategies to deal with negative emotions. 
    \item A set of supervised classifiers of developers' emotions. These include, to the best of our knowledge, the first attempt at classifying arousal during a programming tasks.
    \item A lab package\footnote{\url{https://figshare.com/s/6c13fdc110641872357b}} to verify the results, replicate, and build upon this study.
\end{itemize}

The reminder of the paper is structured as follows.
Section~\ref{sec:background} describes the theoretical model we use to operationalize emotions, reviews  the existing literature on sensor-based emotion detection, and summarizes the empirical studies we build-upon in this work.
In Section~\ref{sec:design}, we describe the design of this study.
In Section~\ref{sec:analysis}, we report the analysis results and answer the research questions.  
In Section~\ref{sec:discussion}, we compare our findings with previous work and discuss their implications and limitations. 
Section~\ref{sec:conclusion} concludes the paper. 


==> tables/enrichedtraining.tex <==
\begin{table}[htb]
\begin{tabular}{llllllp{0.3cm}}
 \multicolumn{6}{c}{\textit{Hold-out setting with enriched train set}} \\
 \hline
 \textbf{Devices} & \textbf{Alg.} & \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{Acc.} & \textbf{St.dev.} \\
 \hline
\multicolumn{6}{c}{\textit{Valence}} \\
 Full set & mlp & .73 (+.05) & .70 (+.10) & .71 (+.11) & .76 (+.05) & .09 \\
 Brainlink & j48 & .54 (+.08) & .52 (--) & .49 (-.02) & .67 (+.01) & .08 \\
 Empatica & rf & .66 ('.04) & .63 (+.04) & .63 (+.04) & .71 (--) & .14 \\
 \hline
 \multicolumn{6}{c}{\textit{Arousal}} \\
 Full set & Jrip & .57 (+.02) & .57 (-.05) & .56 (-.04) & .61 (-.03) & .02 \\
 Brainlink & rf & .55 (+.10) & .56 (-.11) & .55 (-.02) & .59 (-.03) & .10 \\
Empatica & knn & .64 (+.12) & .62 (-.03) & .59 (+.04) & .68 (+.03) & .12 \\
\hline
\end{tabular}
\caption{Performance for the best  machine  learning  classifiers for Valence and Arousal in the Hold-out setting with train set enriched with measurements from the emotion-elicitation step. In parenthesis, we indicate the delta with respect to the hold-out setting reported in Table~\ref{tab:machineLearning}}
\label{tab:enrichedTrainSet}
\end{table}

==> tables/machinelearning.tex <==
\begin{table*}[htb]
\begin{tabular}{l|lllllp{0.5cm}|llp{0.5cm}}
\cline{2-10}
\multicolumn{1}{c|}{} & \multicolumn{6}{c|}{\begin{tabular}[c]{@{}c@{}}Hold-out setting \\ Train: 90\% + LOO cross validation\\ Test: 10\% (x 10 times)\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}Leave-one-subject out setting\\ Train: all-1 subject + LOO cross validation\\ Test: 1 held-out subject (x 23 subjects)\end{tabular}} \\ \hline
\multicolumn{10}{|c|}{\textit{Valence}} \\ \hline
\textbf{Devices} & \textbf{Alg.} & \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{Accuracy} & \textbf{St. Dev.} & \textbf{Alg.} & \textbf{Accuracy} & \textbf{St. Dev.} \\
\hline
Full set & knn & .68 (+.34) & .60 (+.10) & .60 (+.20) & .72 (+.03) & .12 & svmLin & .69 & .25 \\
Brainlink & rf & .54 (+.20) & .54 (+.04) & .52 (+.11) & .66 (-.02) & .07 & mlp & .71 & .22\\
Empatica & knn & .70 (+.36) & .59 (+.09) & .59 (+.18) & .71 (+.03) & .07& svmLin & .68 & .27 \\
\hline
\multicolumn{2}{l}{\textit{Baseline (majority class)}} & \textit{.34} & \textit{.50} & \textit{.41} & \textit{.68} & \multicolumn{4}{c}{--}\\ \hline
\multicolumn{10}{|c|}{\textit{Arousal}} \\ \hline
Full set & rf & .62 (+.31) & .61 (+.11) & .59 (+.21)  & .65 (+.04) & .05 & svmLin & .61 & .25\\
Brainlink & rf & .66 (+.35) & .59 (+.09) & .58 (+.20) & .63 (+.01) & .12 & nb & .63 & .17\\
Empatica & knn & .67 (+.36) & .58 (+.08) & .55 (+.17) & .65 (+.04) & .10 & J48 & .62 & .25\\
\hline
\multicolumn{2}{l}{\textit{Baseline (majority class)}} & \textit{.31} & \textit{.50} & \textit{.38} & \textit{.62} & \multicolumn{4}{c}{--}\\
\hline
\end{tabular}
\caption{Best classifiers performance for  Valence and Arousal. Improvement over the majority class baseline are reported in parenthesis.}
\label{tab:machineLearning}
\end{table*}

==> tables/table_features.tex <==
\begin{table*}[ht]
%\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{@{}p{1cm}llp{2cm}@{}}
\toprule
     \textbf{Sensor} & \textbf{Signal} & \textbf{Features}            &  \\ 
\midrule                                                                                     
Brainlink & EEG    & \begin{tabular}[c]{@{}l@{}}
                $\bullet$ Frequency bin for alpha, beta, gamma, delta and theta waves\\ 
                $\bullet$ Ratio between frequency bin of each band and one another \\
                $\bullet$ For attention and meditation: min, max, difference between mean for baseline and task task\end{tabular} &  \\
\midrule                                                                                     
    \multirow{9}*{Empatica E4} & EDA tonic  & $\bullet$ mean tonic signal     &  \\
                         & EDA phasic & \begin{tabular}[c]{@{}l@{}}
                         $\bullet$ area under the receiving operator curve (AUC) \\ 
                         $\bullet$ min, max, mean, sum peaks amplitudes\end{tabular} &  \\
%\midrule                     
 %\multirow{3}{*}   {Empatica E4} 
 & BVP   &             
        \begin{tabular}[c]{@{}l@{}}
        $\bullet$ min, max, mean, sum peak amplitudes\\ 
        $\bullet$ mean peak amplitude (difference between  baseline and task)\end{tabular}   &  \\
    & HR    
        & \begin{tabular}[c]{@{}l@{}}$\bullet$ mean heart rate (difference between baseline and task\\ $\bullet$ heart-rate variance (difference between baseline and task\end{tabular} &  \\
    %& \begin{tabular}[c]{@{}l@{}}
 %  HRV\end{tabular} & 
  %      \begin{tabular}[c]{@{}l@{}} 
   %     $\bullet$ standard deviation of beat-to-beat intervals\\ $\bullet$ root mean square of the successive differences \end{tabular} &  \\ 
                              
 \bottomrule
\end{tabular}
\end{center}
%\end{minipage}
\label{tab:features2}
\caption{Machine learning features grouped by physiological signal and by sensor}
\vspace{-5mm}
\end{table*}



